Optimal Subcubic Byzantine Agreement with Plain PKI

We consider Byzantine Agreement (BA), where $n$ parties run a distributed protocol to agree on a common value, despite $t$ parties being byzantine. In the synchronous setting, a choice must be made between the weaker unauthenticated setting, which only allows $t < n/3$ byzantine parties, and the stronger authenticated setting that allows up to $t < n/2$ byzantine parties. For this latter setting, BA can be solved with optimal resiliency and optimal bit complexity. However, so far, all optimal solutions rely on the use of threshold signatures. This shows a gap compared to regular signatures, where only protocols with cubic complexity are known for optimal resiliency $t < n/2$. We wonder whether this cubic complexity is required without the use of threshold signatures and show that this is not the case. More specifically, given $\kappa$ an upper bound on the size of a hash or signature, we describe a deterministic protocol solving BA with bit complexity $\mathcal{O}(\kappa^{(\sqrt{13} - 1)/2} n^{(\sqrt{13} + 1)/2}) \approx \mathcal{O}(\kappa^{1.303}n^{2.303})$ while having optimal resiliency $t<n/2$ and round complexity $\mathcal{O}(n)$.

==> macros.tex <==

%----- Algorithm Environment ----------------------------------
\RequirePackage{algpseudocode}
%Header for Algorithms/Functionalities
\newcommand{\algoHead}[1]{\vspace{0.2em} \underline{\textbf{#1}} \vspace{0.3em}}
\newcommand{\algoHeadExt}[2]{\vspace{0.2em} \underline{\textbf{#1} #2} \vspace{0.3em}}
%Multiline Algo-States
\makeatletter
\algnewcommand{\ExtendedState}[1]{\State
\parbox[t]{\dimexpr\linewidth-\ALG@thistlm}{\hangindent=\algorithmicindent\strut\hangafter=3#1\strut}}
\makeatother
%Algorithms States
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
%Algo Comments
\algrenewcommand{\algorithmiccomment}[1]{{\color{gray}// #1}}
%Inline ifs
\algnewcommand{\IIf}[1]{\State\algorithmicif\ #1\ \algorithmicthen}
\algnewcommand{\EndIIf}{\unskip\ \algorithmicend\ \algorithmicif}
\algdef{SE}[InParallel]{InParallel}{EndParallel}[1]{\textbf{in parallel} #1 \textbf{do}}{}

% Define "upon" keyword in algpseudocode.
\algdef{SE}% flags used internally to indicate we're defining a new block statement
[UPON]% new block type, not to be confused with loops or if-statements
{Upon}
{EndUpon}
[1]% There is one argument.
{Upon {#1}} % How begin looks.
{\textbf{end upon}} % How end looks.
\algtext*{EndUpon} % Remove end, forcefully.
% The proper way to remove them based on package flags.
% \makeatletter
% \ifthenelse{\equal{\ALG@noend}{t}}%
%   %{}
%   {\algtext*{EndUpon}}
%   {}%
% \makeatother

% Define "when" keyword in algpseudocode.
\algdef{SE}% flags used internally to indicate we're defining a new block statement
[WHEN]% new block type, not to be confused with loops or if-statements
{When}
{EndWhen}
[1]% There is one argument.
{When {#1}} % How begin looks.
{\textbf{end when}} % How end looks.
\algtext*{EndWhen} % Remove end, forcefully.
%\algtext*{EndIf} % This was here before for some reason.
% The proper way to remove them based on package flags.
% \makeatletter
% \ifthenelse{\equal{\ALG@noend}{t}}%
%   %{}
%   {\algtext*{EndWhen}}
%   {}%
% \makeatother

%----- Box Environment -----------------------------------------
% v 2019.1.DT small skips
%---
 \RequirePackage{varwidth}
 \RequirePackage{color}
 \RequirePackage[most]{tcolorbox}%with most option


%----- Protocol Boxes
 \newtcolorbox{titlebox}[5]{enhanced,center,colframe=black,colback=white,boxrule={#3},arc={#2},auto outer arc,%
 breakable,pad at break*=5pt,vfill before first,before={%\par\smallskip\noindent
 },after={\par\smallskip},top=12pt,left=4pt,%
 enlarge top by=2pt,%enlarge bottom by=7pt,%
 fontupper=\small,
 title={\rule[-.3\baselineskip]{0pt}{\baselineskip}\normalsize\sffamily\bfseries #1}, varwidth boxed title*=-30pt, 
 attach boxed title to top left={yshift=-10pt,xshift=10pt}, coltitle=black,
 boxed title style={colback=white,boxrule={#5},arc={#4},auto outer arc}
 }

 \newenvironment{systembox}[1]
 {\vspace{\baselineskip}\begin{titlebox}{Functionality \normalfont #1}{2.5pt}{1pt}{3.5pt}{1pt}}
 {\end{titlebox}}

 \newenvironment{protocolbox}[1]
 {\begin{titlebox}{Protocol \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}


 \newenvironment{adaptedprotocolbox}[1]
 {\begin{titlebox}{Adapted protocol \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}
 
 
  \newenvironment{simulatorbox}[1]
 {\begin{titlebox}{Simulator \normalfont #1}{0.5pt}{0.5pt}{2pt}{0.75pt}}
 {\end{titlebox}}
 
  \newenvironment{processbox}[1]
 {\begin{titlebox}{Process \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}

 \newenvironment{algobox}[1]
 {\begin{titlebox}{Algorithm \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}
 
 \newenvironment{funcbox}[1]
 {\begin{titlebox}{Function \normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}

  \newenvironment{dianabox}[1]
 {\begin{titlebox}{\normalfont #1}{0.5pt}{0.5pt}{1pt}{0.75pt}}
 {\end{titlebox}}
